Cycle-Accurate Evaluation of Software-Hardware Co-Design of Decimal Computation in RISC-V Ecosystem

Software-hardware co-design solutions for decimal computation can provide several Pareto points to development of embedded systems in terms of hardware cost and performance. This paper demonstrates how to accurately evaluate such co-design solutions using RISC-V ecosystem. In a software-hardware co-design solution, a part of solution requires dedicated hardware. In our evaluation framework, we develop new decimal oriented instructions supported by an accelerator. The framework can realize cycle-accurate analysis for performance as well as hardware overhead for co-design solutions for decimal computation. The obtained performance result is compared with an estimation with dummy functions.

==> propose.tex <==
The architecture (hardware) and programming model (software) are described in this section. The overall model of the proposed framework is depicted in Fig.~\ref{fig:overall}. 
On the hardware part, necessary FSM and hardware description for the accelerator are designed. Rocket chip is then compiled and built with the newly generated
accelerator and an executable for the emulator is generated. On the other hand, in software part, RISC-V in-line assembly and C source code are compiled by RISC-V GCC cross compiler to generate RISC-V binary. After that, the binaries are simulated by SPIKE ISA
simulator for functional verification. Hereafter RISC-V machine code
is generated to be executed on the emulator. Finally, 
the emulator is executed to get the evaluation output and wave forms. A detailed description of architecture (hardware) and programming model (software) is given below:

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{instruction.pdf}
	\caption{RoCC instruction encoding (number of bits).}
	\label{fig:instruction}
\end{figure}


\begin{table}[t]
\centering
\caption{\riaz{List of instructions}}
\label{tlb:function}
\begin{tabular}{l|l|l}\hline
Function    & \textit{Function7}  & Description                                \\ \hline
%\begin{tabular}[c]{@{}l@{}}WR, RD\\ LD, ACCUM \end{tabular} & 0000000-100  & Write, Read, Load, Accum \\\hline
\texttt{WR} & 0000000 & \begin{tabular}[c]{@{}l@{}}Write a value\\ to a register in Rocket core\end{tabular} \\ \hline
\texttt{RD} & 0000001 & \begin{tabular}[c]{@{}l@{}}Read a value\\ from a register in Rocket core\end{tabular} \\ \hline
\texttt{LD} & 0000010 &  Load a value from a memory\\ \hline
\texttt{ACCUM} & 0000011 &  \begin{tabular}[c]{@{}l@{}}Accumulate a value into a register\\ in Rocket core\end{tabular}\\ \hline
\texttt{DEC\_CNV}   &0000110   & \begin{tabular}[c]{@{}l@{}}Convert binary number to\\ corresponding BCD\end{tabular}\\ \hline
\texttt{DEC\_MUL}   &0000111   & Multiply two BCD numbers               \\ \hline
\texttt{DEC\_ADD}   & 0000100  & Add two BCD numbers                          \\ \hline
\texttt{DEC\_ACCUM} & 0001000  & \begin{tabular}[c]{@{}l@{}}Accumulate BCD numbers stored \\in internal registers\end{tabular}\\ \hline
\end{tabular}
\end{table}


\begin{table*}[t]
\centering
\caption {RoCC instructions (number of bits)}
\label{tlb:instruction}
\begin{tabular}{llllllll}
31                                                                                            & 25                             & 19                            & \multicolumn{3}{l}{15}                                                                                                                                                                                                  & 11                               & 6                                                                                   \\ \hline
\multicolumn{1}{|l|}{Instruction}                                                             & \multicolumn{1}{l|}{Source -1} & \multicolumn{1}{l|}{Source-2} & \multicolumn{3}{l|}{Addressing mode}                                                                                                                                                                                    & \multicolumn{1}{l|}{Destination} & \multicolumn{1}{l|}{Fixed opcode}                                                   \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\texttt{Function7}(7)\\ rocc instruction\end{tabular}} & \multicolumn{1}{l|}{\texttt{rs2}(5)}    & \multicolumn{1}{l|}{\texttt{rs1}(5)}   & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}xd\\ (1)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}xs1\\ (1)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}xs2\\ (1)\end{tabular}} & \multicolumn{1}{l|}{\texttt{rd}(5)}       & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\texttt{Opcode}(7)\\ Custom-0\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{\texttt{CLR\_ALL} (0000101)}                                                       & \multicolumn{1}{l|}{00000}     & \multicolumn{1}{l|}{00000}    & \multicolumn{1}{l|}{0}                     & \multicolumn{1}{l|}{0}                                                 & \multicolumn{1}{l|}{0}                                                 & \multicolumn{1}{l|}{00000}       & \multicolumn{1}{l|}{0010111}                                                       \\ \hline
\multicolumn{1}{|l|}{\texttt{RD} (0000010)}                                                             & \multicolumn{1}{l|}{00000}     & \multicolumn{1}{l|}{01011}    & \multicolumn{1}{l|}{0}                     & \multicolumn{1}{l|}{0}                                                 & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{00000}       & \multicolumn{1}{l|}{0010111}                                                       \\ \hline
\multicolumn{1}{|l|}{\texttt{WR} (0000000)}                                                             & \multicolumn{1}{l|}{00000}     & \multicolumn{1}{l|}{01011}    & \multicolumn{1}{l|}{1}                      & \multicolumn{1}{l|}{0}                                                 & \multicolumn{1}{l|}{0}                                                        & \multicolumn{0}{l|}{00000}      & \multicolumn{1}{l|}{0010111}                                                       \\ \hline
\multicolumn{1}{|l|}{\texttt{DEC\_ADD} (0000100)}                                                       & \multicolumn{1}{l|}{01010}     & \multicolumn{1}{l|}{01011}    & \multicolumn{1}{l|}{1}                      & \multicolumn{1}{l|}{1}                                                 & \multicolumn{1}{l|}{1}                                                       & \multicolumn{1}{l|}{01100}       & \multicolumn{1}{l|}{0010111}                                                       \\ \hline
\end{tabular}
\end{table*}









\subsection{Architectural Design (Hardware)}
\begin{comment}
\begin{enumerate}
\item Configuring co-processor interface.
\item Generating own required configuration using the interface.
\item Define function and operation FSM (state machines): This is the most important part where the state machine is programmed to execute the new instruction. Based on the instruction of each function within the function.
\item Modify core to interduce new interface.
\item Configuring simulator with the new interface.
\item Rum benchmark testing to check the functionality.

\end{enumerate}        
\end{comment}
To embed the decimal arithmetics into a RoCC co-processor, two major parts, interfacing and executing units, are required.
RoCC has three default interface signals and they are:
\begin{enumerate}
\item {Core control (CC): for co-ordination between an accelerator and Rocket core.}
\item {Register mode (Core): for the exchange of data between an accelerator and Rocket core.}
\item {Memory mode (Mem): for communication between an accelerator and L1-D Cache.}
\end{enumerate}
Besides the default interface, there is some extended RoCC interface
like floating-point unit for send and receive data from an FPU and
few more.
The interface between the core and accelerator with default interface signal that communicates through core and memory by the command (\textit{cmd}), response (\textit{resp}). 


Figure~\ref{fig:instruction} shows RoCC 32-bit custom instruction encoding with the bit length of several parts of the instruction.
The opcode is selected from {\textit {custom-0} to \textit{custom-3}} reserved for custom instructions, 
and each opcode realizes several functions using \texttt{function7} bits.
Each instruction can have at most one destination register \texttt{rd} and two source registers \texttt{rs1} and \texttt{rs2}.

Three flags \texttt{xd}, \texttt{xs1}, and \texttt{xs2} specify whether registers
in Rocket core are used as destination or source registers. That is,
these flags show the necessity of synchronization between Rocket core
and the accelerator. If the flag value is 1, a register in Rocket core
is used, that is, the values are transferred with the instruction when
{\tt xs1}=``1'' or {\tt xs2}=``1'' and Rocket core waits for the
response when {\tt xd}=``1'', otherwise, it specifies the address of
the register file in the accelerator or the corresponding field is not
used.


Table~\ref{tlb:function} lists the developed  instructions for decimal arithmetic in the framework.
Though we have already developed some of instructions with dedicated hardware, any such hardware component can be integrated into the design.

The RoCC interface is used to realize communication between Rocket core and the accelerator or between memory (cache) and the accelerator through \textit{cmd} and \textit{resp}. 
The accelerator} receives and decodes the commands from Rocket core.
% and programming flow control. To manage the flow of instruction this module use \textit{ready} signal. 
Depending upon the value of \texttt{function7}, 
the corresponding function is executed.
%it perform checking. 
Table~\ref{tlb:instruction} shows the list of some new instructions used in the framework with corresponding values, where core internal integer register 10 and 11 are used as source registers and 12 is used as the destination register. 
%Execution part performs the execution (read, write and BDC add) of the operation. 
Figure~\ref{fig:backend} shows the high-level
architecture of the accelerator, while Fig.~\ref{fig:fsm} shows the
implementation of the finite state machine required to implement the accelerator.



\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{backend.pdf}
	\caption{Basic block of Method-1 in~\cite{Riaz2018}.}
	\label{fig:backend}
\end{figure}




\begin{figure}[t]
	\centering
	\includegraphics[width=0.85\linewidth]{fsm_m1.pdf}
	\caption{Interface FSM of required function for Method-1 in~\cite{Riaz2018}.}
	\label{fig:fsm}
\end{figure}




\begin{comment}
\begin{lstlisting}[caption={Define new instruction},captionpos=b][h]
val doWrite    = funct === UInt(0) 
val doRead     = funct === UInt(1) 
val doLoad     = funct === UInt(2) 
val doAccum    = funct === UInt(3) 
val doBCDadd   = funct === UInt(4) 
val doBCDaccum = funct === UInt(5)
val doBCDconv  = func  === UInt(6)
val doClear    = funct === UInt(7)
\end{lstlisting}
\end{comment}
%The \textit{function-7} bits define the actual operations done by the accelerator. 

For example,
%when the (CLR\_ALL) instruction is fired,
%all the internal registers are set to zero or 
when (\texttt{DEC\_ADD} instruction is required, it performs BCD
(Binary Coded Decimal) addition for two operands and writes the result
to the destination register.  The pseudo-code written in Chisel for an
instruction \texttt{DEC\_ADD} (\texttt{function7} = ``0000100''}) is as
follows.
\begin{lstlisting} %[caption={Define new instruction},captionpos=b][h]
//function bit definition
val DEC_ADD = funct === UInt(4) 
//specific function call
when(cmd.fire() && (DEC_ADD))
//write the result after add X , Y
regfile(addr) := CLA(cmd.bits.rs1,cmd.bits.rs2)
\end{lstlisting}
When the accelerator receives \texttt{DEC\_ADD} command, it executes
the command by adding values of two source registers \texttt{rs1}
and \texttt{rs2} and then write the result to destination
register \texttt{xd}.  Here CLA (Carry-lookahead adder) performs BCD
add operation.  Once the accelerator design is completed, the new chip
is generated with the new accelerator.

\subsection {Programming Model (Software)}
A set of software programs are implemented for the main algorithm where dedicated functions are used to call new instructions supported by the accelerator.

The fragments of the pseudo-code using
accelerator are as follows:

\begin{lstlisting} %[caption={Define new instruction},captionpos=b][h]
//Multiplicand multiple generation 1X-9X
MM[0]=0; MM[1]=X; 
for ( i = 1; i<9 ; i=i+1){
  //Function call in-line assembly
  DEC_ADD_rocc(MM[i+1],MM[1], MM[i]);
}
\end{lstlisting}


\begin{lstlisting} %[caption={Define new instruction},captionpos=b][h]

//Partial porduct accumulation
for ( j=0; j <64 ; j=j+4){
  DEC_ADD_rocc(product,product,MM[MID(Y_64,j,j+4)]);
  product << 4; // shift one decimal digit
}
\end{lstlisting}


The first fragment is used to generate multiplicand multiple and the
second fragment is for accumulating the partial product to
generate final result (See Fig.~\ref{fig:method-1} on
Sec.~\ref{sec:codesign}).
\textit{DEC\_ADD\_rocc} is a function to call \textit{DEC\_ADD} instruction.
%Here X and Y are the BCD coefficient of multiplicand X and Multiplier Y. 
The function \textit{DEC\_ADD\_rocc} takes two BCD inputs and return
the result after BCD addition.  A set of MACROs and inline assembly programs are used to define the
function \textit{BCD\_ADD\_rocc}.
%Where under the opcode \textit{custom-0} source and destination register along with function number is defined. In the above case the the accelerator first read the source registers \texttt{rs1} and \texttt{rs2} and execute (DEC\_ADD) after that the result are written back to the destination register \texttt{xd}. 
In this example code, MID(A, B, C) is MACRO to extract the specific
bit of A within the range C to B. As both source are in BCD format,
where every  four bit represents one digit, thus in every
cycle of the for loop pick one digit of multiplier and then add
multiplicand multiple to generate the final product.}
% The
%BCD\_rocc function are define in terms of actual assembly instruction
%by using inline assembly.

%Adding custom instruction to RISC-V ISA takes several steps and modification. In that case the instruction can directly use as inline assembly like bellow:

%\begin{lstlisting}
%asm volatile(
%    "DEC_ADD_rocc%[z],%[x],%[y]\n\t"
%    : [z] "=r" (c)
%    : [x] "r" (a), [y] "r" (b)
%    return c;)  
%
%\end{lstlisting}

%On the other hand, if the instruction is not known to the compiler the inline assembly looks like:
The function that calls \texttt{DEC\_ADD} instruction is as follows.
\begin{lstlisting}
int DEC_ADD_rocc(int a, int b, int c) {
  asm __volatile__ (".word0x08A5F617\n");
  return a;
}
\end{lstlisting}
In the code, "0x08A5F617" is the hex value for
instruction \textit{custom-0} (\texttt{DEC\_ADD}),
%According to Table~\ref{tlb:instruction}, where the list of new
%instructions used in Method-1 with corresponding values are listed.
where Rocket internal registers 10 and 11 are used as source registers
and 12 is used as the destination register.  In our framework, we also
provide a set of dynamic MACROs to automatically generate the hex
value of corresponding instruction.


